Topological Neural Networks go Persistent, Equivariant, and Continuous

Topological Neural Networks (TNNs) incorporate higher-order relational information beyond pairwise interactions, enabling richer representations than Graph Neural Networks (GNNs). Concurrently, topological descriptors based on persistent homology (PH) are being increasingly employed to augment the GNNs. We investigate the benefits of integrating these two paradigms. Specifically, we introduce TopNets as a broad framework that subsumes and unifies various methods in the intersection of GNNs/TNNs and PH such as (generalizations of) RePHINE and TOGL. TopNets can also be readily adapted to handle (symmetries in) geometric complexes, extending the scope of TNNs and PH to spatial settings. Theoretically, we show that PH descriptors can provably enhance the expressivity of simplicial message-passing networks. Empirically, (continuous and E(n)-equivariant extensions of) TopNets achieve strong performance across diverse tasks, including antibody design, molecular dynamics simulation, and drug property prediction.

==> table_compare.tex <==
\begin{comment}
    

\begin{table*}[ht]
    \caption{ \textbf{Overview of recent prediction methods for relational data. } }
    \label{tab:comp_table}
    \begin{center}
            \resizebox{0.7\textwidth}{!}{\begin{tabular}{lccccr}
                \toprule
                Method & Equivariant & Persistent & Continuous & Higher-order & \\ \midrule
                TOGL     & \xmark & \cmark & \xmark& \xmark &\citet{horn2021topological}     \\
                PersLay     & \xmark & \cmark & \xmark& \xmark &\citet{carrierePersLayNeuralNetwork2020}     \\
                RePHINE     & \xmark & \cmark & \xmark& \xmark &\citet{rephine}     \\
                %\midrule
                MPSN  & \xmark & \xmark & \xmark & \cmark  &\citet{bodnar2021weisfeiler} \\ 
                CWN  & \xmark & \xmark & \xmark & \cmark  &\citet{Bodnar2021} \\
                CAN  & \xmark & \xmark & \xmark & \cmark  &\citet{giusti2023cell} \\
                %\midrule
                IMPSN     & \cmark & \xmark & \xmark& \cmark  &\citet{eijkelboom2023mathrm}     \\
                EGNN     & \cmark & \xmark & \xmark& \xmark  &\citet{satorras2021n}     \\
                E3NN     & \cmark & \xmark & \xmark& \xmark  &\citet{geiger2022e3nn}     \\
                GATr & \cmark & \xmark & \xmark& \xmark  &\citet{brehmer2023geometric}     \\
                %\midrule
                GRAND & \xmark & \xmark & \cmark & \xmark & \citet{chamberlain2021grand}\\
                GREAD & \xmark & \xmark & \cmark & \xmark & \citet{choi2022gread}\\
                GRAND++ & \xmark & \xmark & \cmark & \xmark & \citet{thorpe2022grand++}\\
                \midrule
                TopNets    & \cmark & \cmark & \cmark &\cmark & this work    \\
                \bottomrule
            \end{tabular}}
    \end{center}
\end{table*}
\end{comment}
\begin{tabular}{lcccc}
                \toprule
                Method & Equivariant & Persistent & Continuous & Higher-order  \\ \midrule
                TOGL~\citep{horn2021topological}      & \xmark & \cmark & \xmark& \xmark     \\
                PersLay~\citep{carrierePersLayNeuralNetwork2020}     & \xmark & \cmark & \xmark& \xmark     \\
                RePHINE~\citep{rephine}     & \xmark & \cmark & \xmark& \xmark     \\
                %\midrule
                MPSN~\citep{bodnar2021weisfeiler}  & \xmark & \xmark & \xmark & \cmark  \\ 
                CWN~\citep{Bodnar2021}  & \xmark & \xmark & \xmark & \cmark  \\
                CAN~\citep{giusti2023cell}  & \xmark & \xmark & \xmark & \cmark  \\
                %\midrule
                IMPSN~\citep{eijkelboom2023mathrm}     & \cmark & \xmark & \xmark& \cmark     \\
                EGNN~\citep{satorras2021n}     & \cmark & \xmark & \xmark& \xmark    \\
                E3NN~\citep{geiger2022e3nn}     & \cmark & \xmark & \xmark& \xmark    \\
                GATr~\citep{brehmer2023geometric} & \cmark & \xmark & \xmark& \xmark    \\
                %\midrule
                GRAND~\citep{chamberlain2021grand}& \xmark & \xmark & \cmark & \xmark\\
                GREAD~\citep{choi2022gread}& \xmark & \xmark & \cmark & \xmark \\
                GRAND++~\citep{thorpe2022grand++} & \xmark & \xmark & \cmark & \xmark\\
                \midrule
                TopNets    & \cmark & \cmark & \cmark &\cmark    \\
                \bottomrule
            \end{tabular}

==> table_contrib.tex <==
\definecolor{forestgreen}{HTML}{008000}

\begin{tcolorbox}[tab2,title=Contributions of this work, boxrule=0.4ex,top=0.9ex,bottom=0.9ex,colbacktitle=lb!15!white,colframe=lb!70!white]
\vspace{-1em}
\begin{align*}
    &\textbf{Unified Framework: TopNets} \quad & \text{Section}~\ref{sec:unify} \\
    &\textbf{TNNs + PH} \succ \textbf{TNNs} &\text{Prop}~3.1 \\
    &\textbf{E(n) E-TopNets} &\text{Section}~\ref{sec:equiv_ph}\\
    &\textbf{No VC... for E(n) E-TopNets} &\text{Prop}~\ref{sec:equiv_ph}\\
    &\textbf{Continuous E-TopNets} & \text{Section}~\ref{sec:unify}\\
    &\textbf{Error Bound with Cont. TOGL} & \text{Prop}~5.1 \\
    &\textbf{Error Bound with Cont. RePHINE} & \text{Prop}~5.2
  \end{align*}
\end{tcolorbox}

==> table_topnets.tex <==
%\resizebox{\columnwidth}{!}{
\begin{tcolorbox}[tab2,title=Steps of a TopNet Layer, boxrule=0.4ex,top=0.9ex,bottom=0.9ex,colbacktitle=lb!15!white,colframe=lb!70!white]
\textbf{General Message Passing (MP):} Let ($K^\ell$, $x^\ell$) denote an attributed simplicial complex at layer $\ell$. TopNets recursively refine the attributed complex using a general TNN layer as 
\begin{align}
K^\ell, x^\ell = \mathrm{TNNLayer}_{\ell}(K^{\ell-1},
x^{\ell-1}).
\end{align}

\textbf{PH Vectorization:} Next, we compute a persistence diagram induced by a filtering function $f^\ell$ followed by a vectorization procedure $\psi$. As a result, we obtain a topological vector representation $r_{\sigma}^{\ell}$ for each simplex $\sigma$ in $K^\ell$:
\begin{equation}
    r_{\sigma}^{\ell}  = \psi(\mathrm{PD}(\sigma; f^{\ell}, x^{\ell}, K^{\ell})) \quad \forall \sigma \in K^\ell.
\end{equation}
We note that the map $\mathrm{PD}$ computes persistence diagrams for all dimensions $i=0, 1, \dots, \mathrm{dim}(K^\ell)$.

\vspace{6pt}
\textbf{Topological aggregation:} For each dimension $i=0, \dots, \mathrm{dim}(K^\ell)$, we combine the PH and MP embeddings of simplices of dimension $i$ applying a so-called topological aggregation function $\mathrm{TopAgg}_i$. We also group the topological vectors using a dimension-wise set pooling operation, i.e.,
\begin{align}
%h_\sigma^{\ell, i} & = x^{\ell}(\sigma) \quad  \forall \sigma \in K_{[i]}^\ell \\
h^{\ell, i} & = \mathrm{TopAgg}_i(\{x^{\ell}_\sigma\}_{\sigma \in K_{[i]}^\ell}, \{r^{\ell}_\sigma\}_{\sigma \in K_{[i]}^\ell}) \\
m^{\ell,i} & = \mathrm{Pool}(\{r^{\ell}_{\sigma}\}_{\sigma \in K_{[i]}^\ell}).
\end{align}

\textbf{Readout:} We then merge the joint PH-MP vectors $h^{\ell, i}$ and the topological embeddings $m^{\ell, i}$ across layers and, subsequently, across dimensions using two interleaved readout functions:
\begin{align}
h^i &= \mathrm{Readout}_{\text{layer}}(\{h^{\ell, i}\}_\ell, \{m^{\ell, i}\}_\ell)\\
h &= \mathrm{Readout}_{\text{dim}}(\{h^i\}_i). \label{eq:complex-level-vec}
\end{align}
\end{tcolorbox}

